A Unifying View of Optimism in Episodic Reinforcement Learning

The principle of optimism in the face of uncertainty underpins many theoretically successful reinforcement learning algorithms. In this paper we provide a general framework for designing, analyzing and implementing such algorithms in the episodic reinforcement learning problem. This framework is built upon Lagrangian duality, and demonstrates that every model-optimistic algorithm that constructs an optimistic MDP has an equivalent representation as a value-optimistic dynamic programming algorithm. Typically, it was thought that these two classes of algorithms were distinct, with model-optimistic algorithms benefiting from a cleaner probabilistic analysis while value-optimistic algorithms are easier to implement and thus more practical. With the framework developed in this paper, we show that it is possible to get the best of both worlds by providing a class of algorithms which have a computationally efficient dynamic-programming implementation and also a simple probabilistic analysis. Besides being able to capture many existing algorithms in the tabular setting, our framework can also address largescale problems under realizable function approximation, where it enables a simple model-based analysis of some recently proposed methods.

==> gergo.tex <==
\input{gmacros}

\section{Introduction}
Reinforcement learning (RL) is one of the most important frameworks for sequential decision-making under uncertainty \citep{sutton,SB18,Sze10}.
In an RL problem, a learning agent interacts with a potentially complex environment through taking a series of actions based on the observed state of the environment. 
Each action they take provides them with some reward, but also takes them to a new state which will determine their future rewards. The aim of the agent is to pick its actions in a way such that the its total rewards are as large as possible on the long run, which is made difficult by the dependence between the actions taken by the learner and the future states that these actions take the agent to.
The learning problem is typically modeled by a Markov Decision Process (MDP, \citealp{Puterman1994}) where the agent does not know the rewards or transition probabilities. 
Dealing with this lack of knowledge about the environment is a crucial challenge in reinforcement learning: as opposed to the well-understood problem of computing  optimal policies in known MDPs, the RL problem tasks the agent with the much harder challenge of having to maximize its rewards \emph{while} learning about the environment. This presents the learner with the classic dilemma of \emph{exploration versus exploitation}: given their current limited knowledge about the environment, should the agent stick to behaviors that proved rewarding in the past (i.e., exploit), or should it venture into less well-understood parts of the world to seek better rewards (i.e., explore)? The performance of algorithms facing this problem is naturally measured in terms of their \emph{regret}, defined informally as the amount of reward lost within a time horizon of $T$ due to the learner having no knowledge of the environment initially. Good learning algorithms are guaranteed to improve their performance as time progresses, which results in their regret growing as a sublinear function of $T$.
Our paper aims to bring about a better understanding of the most popular family of RL algorithms with formal guarantees on their regret: the family of \emph{optimistic reinforcement learning algorithms}.

The maxim of ``optimism in the face of uncertainty'' (OFU) has been arguably the most influential design principle for algorithms addressing the exploration-exploitation dilemma. Optimistic algorithms operate by maintaining a set of statistically plausible models of the world, and planning their actions in a way that they maximize the returns in the best of the plausible worlds. Such algorithms were first proposed in the simple reinforcement-learning problem of multi-armed bandits by \citet{LaiRo85} and further developed by \citet{Agr95}, \citet{BuKa96} and \citet{auer2002finite}---we refer to the recent monograph of \citet{LSz19book} for an excellent overview. The OFU principle has also inspired numerous reinforcement learning algorithms, starting with the classic RMAX algorithm first proposed by \citet{BraTen02} and further analyzed by \citet{KakadeThesis:2003} and \citet{SziSze10}. Consequently, the past decade saw a series of breakthroughs in reinforcement-learning theory thanks to development of more and more sophisticated optimistic RL algorithms, particularly in the context of regret minimization.


A closer look at the literature reveals two main approaches to incorporating optimism in the setting of reinforcement learning in MDPs. In the first, optimism is introduced through estimates of the MDP: these approaches build a set of plausible MDPs by constructing confidence bounds around the empirical transition and reward functions, and following the policy that grants the highest total expected reward in the best MDP in the set. A representative member of this family of methods is the UCRL2 method of \citet{jaksch2010near}, a variant of the ``Model-Based Interval Estimation'' (MBIE) algorithm of \citet{SL08}. While conceptually appealing, methods that are defined in terms of sets of MDPs tend to be difficult to implement and virtually impossible to reconcile with empirically successful methods.
Another approach to incorporate optimism in RL is through constructing upper bounds on the \emph{optimal value functions} which (roughly speaking) measure the total expected reward of the optimal policy in the true MDP. The resulting estimates are then used to define an optimistic policy that picks its actions to greedily maximize the optimistic values. This approach is taken in the recent works of \citet{azar2017minimax} and \citet{DLB17}, whose respective algorithms UCB-VI and UBEV are variations on another algorithm of \citet{SL08} called ``Model-Based Interval Estimation with Exploration Bonus'' (MBIE-EB). Algorithmically, these methods make use of exploration bonuses added to the reward functions and computing the optimistic value functions via dynamic programming techniques (cf.~\citealp{Ber07:DPbookVol2}), and thus they are much more compatible with mainstream RL algorithms that are typically based on value functions. One downside of these methods is that their probabilistic analysis is often far more complicated than that of methods that work in the space of MDPs\footnote{We invite the reader to take a glimpse at the definition of event $\mathcal{E}$ in Appendix~B.1 of \citet{azar2017minimax} or that of event $F$ in Appendix~E.2 of \citet{DBL17} to verify this.}.



While these two approaches may look very different on the surface, we show in this paper that there is in fact a very strong connection between them. 
In particular, our main contribution is designing a general linear program (LP) formulation of optimistic planning over a set of MDPs, and showing that the corresponding dual linear program induces an optimistic planning problem in the space of value functions. This implies that that for every approach defined in the space of MDPs, there exists an equivalent approach which is optimistic in the space of value functions \emph{and can be implemented via dynamic programming}. This observation removes a long-standing limitation of such algorithms, finally making them compatible with the most common tools of mainstream RL based on value functions \redd{[[maybe some examples?]]}. Besides opening this new avenue of implementation for optimistic algorithms, we also demonstrate that our primal-dual LP perspective significantly facilitates the analysis of the derived RL algorithms. Specifically, we will argue that probabilistic statements can be conveniently handled in the primal space of MDPs, whereas algebraic parts of the analysis are straightforward to tackle in the dual space of value functions through bounding the width of the confidence intervals in this latter space. We will demonstrate this argument by introducing a novel confidence set of MDPs that yields a practical algorithm achieving optimal regret bounds for episodic MDPs. For ease of exposition, we focus on finite-horizon episodic MDPs, but remark that many of our core contributions also generalize to the infinite-horizon average reward case as well.

\redd{[[[Not sure what we mean here:]]] Through strong duality, we are also able to show surprising relationships between existing algorithms that were previously thought to be entirely distinct. We also show how by considering the dual problems, we can gain additional insights into the structure of the confidence sets and optimal policies which in turn can inspire new algorithmic advances.}

The remainder of the paper is organized as follows. In Section~\ref{sec:prob} we formally define the episodic reinforcement learning problem we consider, and in Section~\ref{sec:lps} define the linear programming formulations of two common algorithms, UCRL2 \citep{jaksch2010near}, and UCB-VI \cite{azar2017minimax}. Then in Section~\ref{sec:dual}, we start to consider the duals of these LPs and show some of the additional insights that can be gained from this formulation. In Sections~\ref{sec:ucrlbern,sec:ucrlnew}, we consider variants of UCRL2 which have lower regret, and show that the decrease in regret can be observed by considering the dual problem. {\color{red} this probably isn't the best way to explain this} Finally in Section~\ref{sec:conc} we summarize our results and present directions for future work.
{\color{red} also add somewhere that our method allows us to analyze why some algorithms perform better than others}

\section{Preliminaries on online learning in Markov decision processes}
We begin by defining basic notation and concepts related to finite-horizon episodic Markov decision processes, formulating our learning problem, and describing the classic linear-program formulation of optimal control in MDPs. All statements in this section are standard, and we generally refer the reader to \citet{Puterman1994} for the proofs.
A finite episodic Markov decision process (MDP) is defined as a tuple $(\cS, \cA, H, \alpha, P, r)$ where 
\begin{itemize}
 \item $\cS$ is the finite set of all states, 
 \item $\cA$ is the finite set of actions, 
 \item $H$ is the (fixed) episode length, 
 \item $\alpha$ is the distribution of the initial state in each episode,
 \item $P$ is a the transition function giving the probability $P_h(x'| x,a)$ of reaching state $x'$ after playing action $a$ from state $x$ at step $h$ of an episode, and 
 \item $r_h$ is a reward function that assigns a real-valued reward to each state-action pair. For simplicity of exposition, we will consider deterministic reward functions taking values in $[0,1]$. 
\end{itemize}
We will consider an online learning setting where a learning agent and its environment interact in a sequence of $K$ episodes. At the beginning of each episode $k=1, \dots, K$, an initial state $x_{1,k}$ is sampled from $\alpha$. In subsequent stages $h=1,2,\dots,H-1$ within the episode, the agent observes the state $x_{h,k}$, selects action $a_{h,k}$, earns reward $r_{h,k} = r(x_{h,k},a_{h,k})$, and moves to the next state $x_{h+1,k}\sim P_h(\cdot|x_{h,k},a_{h,k})$. It will be useful to define a \emph{policy} $\pi$ as a mapping from states to actions, $\pi: \cS \to \cA$, and a collection $\bpi = \{\pi_h\}_{h=1}^H$ of policies for each stage $h$ of an episode, since it is known that such collections of policies are sufficient for the purpose of maximizing reward within each episode. We will often simply refer to a collection of policies $\bpi$ as a policy, and also use $T=KH$ to define the total number of rounds. 

\paragraph{Value functions and dynamic programming.} For any policy $\bpi$, we can define the \emph{value function} at each state $x \in \cS$ and each stage $h$ as the expected total reward resulting from running policy $\bpi$ from that point on:
\[
V_h^{\pi}(x) = \E_{\bpi}\bigg[ \sum_{l=h}^H r_l(x_l,\pi_l(x_l)) \bigg| x_h = x \bigg].
\]
We use the notation $\bpi^*$ to denote an \emph{optimal policy} satisfying $V_h^{\pi^*}(x) = \max_{\pi} V_h^{\pi}(x)$ and denote the corresponding \emph{optimal value function} as $V_h^*(x) = V_h^{\pi^*}(x)$ for all $x,h$.  
Analogously to the value functions defined above, we also define the \emph{action-value function} and \emph{optimal action-value function} for each $x,a,h$ as
\[
 Q_h^{\pi}(x,a) = \E_{\bpi}\bigg[ \sum_{l=h}^H r_l(x_l,\pi_l(x_l)) \bigg| x_h = x , a_h = a\bigg] \qquad\mbox{and}\qquad Q_h^{\pi^*}(x,a) = \max_{\pi} Q_h^{\pi}(x,a).
\]
It is easily shown that the value functions satisfy the \emph{Bellman equations} for all $x,a,h$:
\begin{align*}
\begin{aligned}
&V _h^{\pi}(x) = Q_h^{\pi}(x,\pi(x)) 
\\ &Q_h^{\pi}(x,a) = r_h(x,a) + \sum_{y \in \cS} P(y|x,a)V_{h+1}^{\pi}(y)
\\ &V_{H+1}^{\pi}(x) = 0
\end{aligned}
\quad \text{ and } \quad
\begin{aligned}
&V _h^*(x) = \max_{a \in \cA} Q_h^*(x,a)
\\ &Q_h^*(x,a) = r_h(x,a) + \sum_{y \in \cS} P(y|x,a)V_{h+1}^*(y)
\\ &V_{H+1}^*(x) = 0.
\end{aligned}
\end{align*}
It is easy to see that the total expected reward of the optimal policy $\bpi^*$ is $\sum_x \alpha(x) V_1^*(x)$, and an optimal policy can be found by solving the above system of equations by backward recursion through the stages $H,H-1,\dots,1$, a method commonly known as \emph{dynamic programming} \citep{Ber07:DPbookVol2}.
 \redd{[Make $x_1$] deterministic for simplicity?]}
 
\paragraph{Occupancy measures and linear programming.} An alternative (but somewhat less known) method for finding optimal policies is through the following \emph{linear program} formulation (originally due to \redd{[[[Denardo...]]]}). Defining $\cZ = \cS\times\times\cA\times\cS$ and the \emph{occupancy measure} $q^{\bpi}$ of policy $\bpi$ at the state-action-next-state tuple $x,a,x'\in\cZ$ as \redd{[[define notation $\PPcc{\cdot}{\bpi,P}$]]}
\[ 
q^{\bpi}_h(x,a,x') = \PP\left[x_h =x, a_h=a, x_{h+1}=x'\middle|\bpi,P\right],
\]
it is easy to see that the total expected reward of a policy $\bpi$ can be written as
\[
 \sum_x \alpha(x) V^{\bpi}_1(x) = \sum_{h=1}^H \sum_{x,a,x'} q_h^{\bpi}(x,a,x') r(x,a),
\]
which is a linear function of the occupancy measure $q^{\bpi}$. This suggests that the problem of maximizing the expected reward can be reformulated as maximizing the expectation above. It is straightforward to show that the set of occupancy measures is uniquely defined by the following set of \emph{linear} constraints:
\begin{align}
&\redd{q_h(x,a,x') = P(x'|x,a) \sum_y q_h(x,a,y)} \qquad \forall (x,a,x')\in\cZ, \,h=1,\dots,H \label{eq:consistent}
\\ &\sum_{x' \in \cS} \sum_{a \in \cA} q_h(x,a,x') = \sum_{x^- \in \cS} \sum_{a \in \cA} q_{h-1}(x^-,a,x) \qquad \forall x \in \cS,\,h=1,\dots,H \label{eq:flow}
\\ & q_h(x,a,x') \geq 0 \qquad \forall x,x' \in \cS, a \in \cA, \,h=1,\dots,H \label{eq:nonneg}
\\ & \sum_{a \in \cA} \sum_{x' \in \cS} q_1(x,a,x') = \alpha(x) \qquad \forall x \in \cS. \label{eq:initial}
 \end{align}
 The first constraint requires $q$ to respect the dynamics of the MDP, in that the joint distribution $q(x,a,x')$ should match the decomposition $P(x'|x,a) q(x,a)$.
 The second constraint is a \emph{flow constraint} that ensures that the probability of moving into any state (by taking any action from any previous state) is equal to the probability of leaving that state (by taking any action and then moving into any other state). The remaining constraints respectively ensure that 
 states that the occupancies in the first stage correspond to the initial-state distribution $\alpha$ and that the entries of $q_h$ are nonnegative. We will refer to the set of occupancy measures satisfying constraints~\eqref{eq:flow}--\eqref{eq:initial} as the \emph{flow polytope} and will denote it by $F$.
 It is easily seen that constraints~\eqref{eq:flow}--\eqref{eq:initial} together imply that $q_h$ at any stage defines a valid probability distribution over $\cS\times\cA\times\cS$: $\sum_{x,a,x'} q_h(x,a,x') = 1$ (for a proof, see Lemma~\ref{lem:flow} in Appendix~\ref{}). Thus, denoting the set of occupancy measures corresponding to the transition function $P$ by $\Delta(P)$, we can see that the problem of maximizing the total expected reward can be written as the linear program
\redd{[[[Should we index $q$ by $h$? we seem to do that later... New notation $\Delta(P)$ looks more practical.]]]}
\begin{equation}\label{eq:primalMDP}
 \underset{q \in \Delta(P)}{\text{maximize}}  \sum_{h=1}^H \sum_{x,a,x'} q_h(x,a,x')r(x,a).
\end{equation}
An optimal policy $\bpi^*$ can be extracted from the solution $q^*$ of the above problem by observing that every occupancy measure $q$ induces a \emph{stochastic policy} $\bpi^q$ defined as
\[
\pi^q(a|x) = \frac{ \sum_{x' \in \cS} q(x,a,x')}{\sum_{a' \in \cA} \sum_{x' \in \cS} q(x,a',x')},
\]
for all states $x$ where the denominator is nonzero and defined arbitrarily otherwise, where $\pi(a|x)$ gives the probability of taking action $a$ in state $x$. Indeed, the policy $\bpi^{q^*}$ can be shown to be optimal.

\paragraph{Bridging dynamic programming and linear programming.} The linear-programming view we just presented above is closely connected to the dynamic-programming view relying on the definition of value functions. Indeed, by appealing to standard results on LP duality, we can obtain the dual linear program of the LP~\eqref{eq:primalMDP} as
 \begin{equation}\label{eq:dualMDP}
  \begin{split}
\underset{v}{ \text{minimize}} \quad &\sum_{x \in \cS} \alpha(x)v_1(x)
 \\ \text{ subject to } \quad & v_{h}(s) \geq r(x,a) + \sum_{y \in \cS} P(y|x,a) v_{h+1}(y) \qquad \forall x \in \cS, a \in \cA, h = 1,\dots,H.
  \end{split}
 \end{equation}
The solution of the above linear program is easily seen to be the optimal value function $V^*$.





\paragraph{Regret minimization in MDPs.}
Our main focus in this paper is on designing algorithms that learn by sequential interaction in a fixed MDP in a sequence of episodes $k=1,2,\dots,K$. The goal of the learning agent is to pick a sequence of policies $\bpi_{k}$ in each episode $k$ so that its total expected reward gathered during the learning procedure is as large as possible. The key challenge for the learner is that it has \emph{no prior knowledge} of the MDP, so it has to learn about the parameters of the environment while attempting to maximize its reward. The performance of the learner will be measured in terms of its \emph{regret} defined using the notation introduced in the previous section as 
\[
\Reg_T = \sum_{t=1}^K ( V^*_1(x_{1,t}) - V_1^{\bpi_k}(x_{1,t})),
\]
where $T=KH$ is the total number of rounds. \redd{[[[maybe put a summary of existing results here?]]]}

\section{A linear programming framework for optimistic RL algorithms}
This section presents our main contribution of proposing a general linear-programming framework for designing and analyzing optimistic reinforcement-learning algorithms. Our LP framework naturally extends the linear programs~\eqref{eq:primalMDP} and~\eqref{eq:dualMDP} to account for any \emph{uncertainty} that a learner may have about the MDP. The core idea is to express uncertainty in the space of occupancy measures through the use of confidence intervals for the transition functions, and phrase the optimistic planning problem as maximizing the rewards over the resulting set. Our key result will be showing that the dual of this LP can be equivalently written as a dynamic programming problem with added bonuses for exploration.

Our uncertainty sets over occupancy measures will be defined with the help of confidence intervals around a reference transition probability function $\wh{P}$. As a concrete example, consider the confidence sets used by the UCRL2 algorithm of \citet{jaksch2010near} are defined as the set of transition functions $\tP$ satisfying $\bigl\|\tP(\cdot|x,a) - \wh{P}(\cdot|x,a)\bigr\|_1 \le \varepsilon(x,a)$ for all $x,a$ and some appropriately chosen function $\varepsilon\ge 0$. For the sake of flexibility, we will consider more general confidence sets based on the statewise deviations $|\tP(x'|x,a) - \wh{P}(x'|x,a)|$. Specifically, our general constraints on $\tP$ will be expressed in the form 
\begin{equation}\label{eq:aggregation}
\sum_{x'} w_i(x') \bigl|\tP(x'|x,a) - \wh{P}(x'|x,a)\bigr| \le b_i(x,a) 
\end{equation}
for a set of appropriately defined \emph{constraint-aggregation functions} $w_i$ and \emph{confidence widths} $b_i$. For instance, the $\ell_1$ constraints used by UCRL2 can be expressed by choosing a the pair of constant functions $w_i = 1$ and $b_i=\varepsilon$ (cf.~Section~\ref{sec:ucrl}). The aggregation functions will be indexed by the set $\cI$. The true potential of aggregation functions to obtain more sophisticated algorithms will be demonstrated in Sections~\ref{sec:bernstein} and~\ref{sec:subset}.

With these ideas in mind, we define our primal optimistic linear program (POLP) in its general form as follows:
\begin{align}
& \underset{q\in F,\, \varepsilon\in\real_+^{\cZ}}{\text{maximize}} \sum_{x',a,x,h} q_h(x',a,x)r(x,a) & \label{eqn:optlp-primal}
\\ & \text{subject to} \nonumber
\\ & q_h(x,a,x') - \hP(x'|x,a) \sum_{y \in \cS} q_h(x,a,y) \leq \varepsilon_h(x,a,x') & \forall (x,a,x')\in\cZ, h\in[H] \label{eqn:qconst1}
\\ & \hP(x'|x,a) \sum_{y \in \cS} q_h(x,a,y) - q_h(x,a,x') \leq \varepsilon_h(x,a,x')&  \forall (x,a,x')\in\cZ, h\in[H] \label{eqn:qconst2}
\\ & \sum_{y \in \cS} w_{i}(y) \varepsilon_h(x,a,y) \leq b_{i}(x,a) \sum_{y \in \cS} q_h(x,a,y) &\forall i\in\cI,\,(x,a)\in\cS\times\cA, h\in[H] 
\hspace{-.1cm}\label{eqn:epsconst}
\end{align}
To interpret the above constraint, it is helpful to think of the transition model $\tP^q(x'|x,a) = \frac{q(x,a,x')}{\sum_y q(x,a,y)}$ induced by the feasible occupancy measure $q$. We can generally show that the constraints in the space of transition functions $\sum_{x'} w_i(x') \bigl|\tP(x'|x,a) - \wh{P}(x'|x,a)\bigr| \le b_i(x,a)$ are equivalent to the constraints~\eqref{eqn:epsconst}:
\begin{lemma}\label{lem:PvsQ}
 ...
\end{lemma}
Our key technical result is the following theorem that characterizes the dual of the linear program given above.
\begin{theorem}\label{thm:main}
There exists a function $\text{CB}: \cS\times\cA\times[H]\ra\real_+$ such that the dual of the linear program given in Equations~\eqref{eqn:optlp-primal}--\eqref{eqn:epsconst} can be written as
\begin{align}
\underset{v}{\text{minimize}}  \;& \sum_{x \in \cS} \alpha(x)\beta_0(x)&   \label{eqn:lpdualgen}
 \\ \text{ subject to } \;& \nonumber
  \beta_{h}(x) \geq r(x,a)+ \text{CB}_{h}(x,a)  + \sum_{y \in \cS} \hP(y|x,a) \beta_{h+1}(y)  & \forall (x,a)\in\cS\times\cA, h\in[H]. \nonumber
\end{align}
Furthermore, letting $\beta^*$ be the optimal solution of the dual LP above, the optimal policy $\bpi^+$ extracted from any optimal solution $q^*$ of the primal LP satisfies 
\begin{equation}\label{eq:optpolicy}
 \beta^*_{h}(x) = r(x,\pi^+(x))+ \text{CB}_{h}(x,\pi^+(x))  + \sum_{y \in \cS} \hP(y|x,\pi^+(x)) \beta_{h+1}^*(y)  \qquad \forall x\in\cS, h\in[H].
\end{equation}
\redd{[[[don't know how to write this better...]]]}
Finally, if the true transition function $P$ satisfies the constraint in Equation~\eqref{eq:aggregation}, the optimal solution $\beta^*$ of the dual LP satisfies $V^*_h(x) \le \beta^*_h(x) \le H-h$ for all $x\in\cS$.
\end{theorem}
We refer to the above linear program as the Dual Optimistic Linear Program (DOLP).
This LP bears a striking similarity with the dual LP~\eqref{eq:dualMDP} that specifies the optimal value functions in the true MDP, with the key difference being that the reward function $r$ is replaced by the \emph{augmented reward function} $r + \CB$, while the transition function being used is the reference $\hP$. The function $\CB$ can be interpreted as an exploration bonus that drives optimistic exploration directly in the space of value functions. Indeed, another remarkable feature of the above theorem is that it directly shows that the optimal solution $\beta^*$ acts as an upper-confidence bound on the true value function $V^*$ if $P$ satisfies the primal constraints.
It is worth noting that the actual values of $\CB_h$ takes in stage $h$ depend on the constraint-aggregation functions $w_{i,h}$ and $b_{i,h}$ and also on the optimistic value estimates $\beta^*_{k}$ corresponding to future stages $k>h$. This implies that the solution of the LP~\eqref{eqn:lpdualgen} can be found by means of dynamic programming using the reference transition function $\hP$.

To help appreciate the result above, let us draw comparison with the recently proposed methods of \citet{azar2017minimax} and \citet{DLB17} that are based on computing optimistic value functions that can be written as optimal solutions of an LP of the form
\begin{align}
 \underset{v}{\text{minimize}} \;& \sum_{x \in \cS} \alpha(x)v_0(x)& \label{eqn:lpucbvi}
 \\ \text{ subject to } \;& v_{h}(x) \geq r(x,a) + B_{h}(x,a) + \sum_{y \in \cS} \hP(y|x,a) v_{h+1}(y)   & \quad \forall(x,a)\in\cS\times\cA, h\in[H].  \nonumber
 \\ & v_{h}(x) \leq H & \qquad \forall x \in \cS, h\in[H] \nonumber,
 \end{align}
 for some exploration-bonus function $B$. Except for the last constraint (which is automatically satisfied in our LP) and the choice of the exploration bonuses, these algorithms can be seen to be identical to the dynamic-programming methods resulting from our approach. The choice of the bonuses $B$ are carefully chosen to ensure that the resulting solutions are indeed optimistic estimates of the true optimal value function. However, the probabilistic analysis required to show these properties arguably tends to be rather cumbersome, as testified by the sheer number of failure events that the analyses of \citet{azar2017minimax} and \citet{DLB17} require. On the other hand, our approach only requires to ensure feasibility in the primal space of MDPs, which is significantly simpler to reason about.

Indeed, the simplicity of our framework enables us to derive very general algorithms with their corresponding regret bounds given in a straightforward way. 
To this end, we consider algorithms that make use of the dual LP in each episode $t=1,2,\dots,K$ by setting appropriate aggregation functions $w_t$ and $b_t$ capturing the uncertainty about $P$ in episode $t$, and computing optimistic value function $\beta^*_{t}$  by dynamic programming. Having computed this function, the algorithm will follow policy $\pi_t$ satisfying condition~\eqref{eq:optpolicy}. Introducing the notation $\text{CP}_{h,t}(x_{h,t},\pi_t(x_{h,t})) = (\hat P^{\pi_t}_t - P) \beta_{h+1,t}^*$, the regret of this algorithm satisfies the following bound:\redd{[[[maybe write out the definition of \CP\, more properly?]]]}
\begin{proposition} \label{prop:reggen}
On the event $\cap_{t=1}^K \{P \in \cP_t\}$, the regret can be bounded with probability at least $1-2\delta$ as
\[
\Reg_T \leq \sum_{t=1}^K \sum_{h=1}^H \text{CB}_{h,t}\pa{x_{h,t},\pi_t(x_{h,t})} 
+ \sum_{t=1}^K \sum_{h=1}^H \text{CP}_{h,t}\pa{x_{h,t},\pi_t(x_{h,t})}+ 2H\sqrt{2T\log(1/\delta)}\redd{(??)} 
\]
\end{proposition}
\redd{[[[can we improve the last term by using Bernstein's ineq?]]]}
The second sum in the above bound is typically of the same order as the first one. \redd{[[[can we say something stronger?]]]}
This proposition highlights that regret analyses can be decomposed into two main parts: conducting a probabilistic analysis that ensures that the true model lies in the primal feasible set, and upper-bounding the sum of the confidence bonuses. This greatly simplifies the probabilistic analysis as opposed to methods like UCB-VI and UBEV that work in the space of value functions, and also facilitates the analysis related to the confidence widths that is typically more involved for primal-only algorithms like UCRL2. In the following sections, we demonstrate the power of this approach by deriving performance bounds for some old and new algorithms.

Before presenting these algorithms, let us define some notations that we'll be using throughout. The number of times the triple $(x,a,x')$ has been observed up to the end of episode $t$ is denoted as $N_{t}(x,a,x')$, and $N_{t}(x,a)$ is defined similarly for each pair $(x,a)$. Also defining $N_{t}^+(x,a) = \max\ev{N_{t}(x,a),1}$, the reference transition function the algorithms will use is defined as $\hP_{t}(x'|x,a) = \frac{N_{t}(x,a,x')}{N_{t}^+(x,a)}$. We will denote the set of probability distributions over any finite set $\mathcal{X}$ as $\Delta_\cX$ and the set of valid transition functions as $\Delta_{\cS|\cS,\cA}$. All algorithms are based on uncertainty sets derived from concentration inequalities; we use $\delta>0$ to refer to the failure probability of these probabilistic inequalities. \redd{[[[put more common notation here]]]}


\subsection{UCRL2 as optimistic dynamic programming}\label{sec:ucrl}
We begin by describing the influential UCRL2 algorithm of \cite{jaksch2010near} in our framework. In its original form, UCRL2 works in the space of MDPs by specifying a confidence set of transition functions, stated in terms of the $\ell_1$ distance from the empirical transition function:
\[
 \cP_{t} = \{ p \in \DeltaSSA: \; \bigl\| p(\cdot| x,a) -\hP_{t}(\cdot | x,a) \bigr\|_1 \leq \varepsilon_{t}(x,a) \;\;\; (\forall x \in \cS, a \in \cA, h\in[H]) \}
\]
The confidence bounds $\varepsilon_{t}$ are defined using concentration results on the $\ell_1$ norm due to \cite{weissman2003inequalities} and are given up to a constant factor $C$ as
\begin{align*}
\varepsilon_{t}(x,a) &= \sqrt{\frac{CS \log(A/\delta)}{N^+_{t}(x,a)}}
\end{align*}
for all $x\in \cS,a \in \cA$ and time steps $t$. In each round $t$, UCRL2 computes the solution to the optimization problem
\[
 \pa{\bpi_t,\tP_t} = \argmax_{\pi,\tP\in\cP_t} \EEc{V^{\bpi}(x_1)}{\bpi,\tP}.
\]
\redd{[[[does this notation make sense???]]]} By Lemmma~\ref{lem:PvsQ}, this optimization can be seen to be equivalent to solving either of our linear programs~\eqref{eq:primalMDP} or \eqref{eqn:lpdualgen} when choosing the single constant aggregation function $w_i = 1$ and confidence width $b_i = \varepsilon_{t}$. The original implementation of UCRL2 relies on defining an ``extended MDP'' with a continuous action set corresponding to the confidence sets, and solving it by an adaptation of the classic value iteration algorithm called ``extended value iteration'' (see also \citet{neu12ssp} for a version adapted to the episodic case).
Theorem~\ref{thm:main} implies that UCRL2 can be equivalently implemented through a much more straightforward dynamic-programming procedure, using the empirical transition function $\hP_t$ and adding some exploration bonuses $\CB_t$ to the reward function. 
Our main result in this section is providing an explicit form of these exploration bonuses:
\begin{proposition}\label{prop:ucrlbonus}
 The exploration bonus $\CB_{h,t}$ induced by UCRL2 is
 \[
  \CB_{h,t}(x,a) = \frac 12 \pa{\max_{x'} \beta^*_{h+1,t}(x') - \min_{x'} \beta^*_{h+1,t}(x'))}\cdot \varepsilon_{t}(x,a).
 \]
\end{proposition}
Notably, in each stage $h$, the exploration bonuses explicitly depend on the \emph{span} of the optimistic value functions in the next stage $h+1$. Since the property $\beta^*_{h,t}\le H$ holds by Theorem~\ref{thm:main}, we can see that the exploration bonus of UCRL2 is upper-bounded by $H\varepsilon_{h,t}(x,a)$. It is worthwhile to contrast this with the exploration bonus used by the basic version of UCB-VI (UCB-VI-CH, \citealp{azar2017minimax}), written as $H\varepsilon_{h,t}(x,a)/\sqrt{S}$ in our notation. This clearly illustrates the colloquially well-known fact that, in the worst case, the confidence bounds used by UCRL2 tend to be wider than necessary for the sake of regret minimization. We note however that, since the confidence bonuses depend on the actual optimistic value functions, they can be sometimes tighter than the UCB-VI bonuses.

The regret of UCRL2 is, of course, well understood in the episodic setting we consider. Still, we find it instructive to state its regret bound and prove it using the general analytic tool of Proposition~\ref{prop:reggen}, thus demonstrating its utility in a simple setting. Specifically, we prove the following statement on the performance of UCRL2:
\begin{proposition}
 The regret of UCRL2 satisfies
 \[
  \Reg_T \le \redd{C}HS\sqrt{AT} + 2H\sqrt{2T\log(1/\delta)}.
 \]
\end{proposition}
\begin{proof}
 The proof is extremely simple given Proposition~\ref{prop:reggen}. First off, note that by Proposition~\ref{prop:ucrlbonus} and using that $\beta^*_{h,t}\le H$, the exploration bonuses can be bounded as $\CB_{h,t}(x,a)\le H\varepsilon_{h,t}(x,a)$ for all $h,x,a$. Furthermore, we also have
 \begin{align*}
  \CP_{h,t}(x,a) &= \sum_{x'} \bpa{\hP_t(x'|x,a) - P(x'|x,a)} \beta_{h+1,t}^*(x') \le \onenorm{\hP_t(x'|x,a) - P(x'|x,a)} \infnorm{\beta_{h+1,t}^*} 
  \\
  &\le H\varepsilon_{h,t}(x,a).
 \end{align*}
  Thus, using the definition of $\varepsilon_{h,t}$ and Proposition~\ref{prop:reggen}, introducing the notation $C' = \sqrt{C\log(SA/\delta)}$, we can bound the key terms in the regret as
\begin{align*}
&\sum_{t=1}^K \sum_{h=1}^H \text{CB}_{h,t}\pa{x_{h,t},a_{h,t})} + \sum_{t=1}^K \sum_{h=1}^H \text{CP}_{h,t}\pa{x_{h,t},a_{h,t}} 
\\
&\le 2H\sum_{t=1}^K \sum_{h=1}^H \varepsilon_{h,t}\pa{x_{h,t},a_{h,t}} = 
2 C'H \sum_{t=1}^K \sum_{h=1}^H \sum_{x,a} \II{\pa{x_{h,t},a_{h,t})} = (x,a)} \sqrt{\frac{S}{N^+_{t}(x,a)}}
\\
&\stackrel{(a)}{\le} 4C'H \sum_{x,a} \sqrt{S N_{K}(x,a)} 
\stackrel{(b)}{\le} 
4C'H S\sqrt{A \sum_{x,a} N_{K}(x,a)}
\\
&\stackrel{(c)}{=} 4C'H^{3/2} S\sqrt{AK} = 4C'HS\sqrt{AT},
\end{align*}
where step ($a$) uses a pigeon-hole argument, step $(b)$ uses Jensen's inequality, and step $(c)$ uses the fact that $\sum_{x,a} N_{K}(x,a) = KH$.
Setting $C' = ...$ guarantees that the event $\cap_{t=1}^K \{P \in \cP_t\}$ holds with probability $1-\delta$ due to...
\end{proof}
A well-known limitation of UCRL2 is that its best known regret bound is suboptimal in terms of both $H$ and $S$, as the minimax regret in the problem we consider is known to be of order $\sqrt{HSAT}$. As expected, our analysis does not improve this bound either. To address this issue, we derive new algorithms using our optimistic LP framework that improve these dependencies in the next sections.






\subsection{Optimistic linear programming with empirical Bernstein confidence bounds}
In this section, we use our framework to define a new algorithm that uses empirical Bernstein inequalities for quantifying uncertainty in the space of transition functions. 
Through analysis of the dual LP, we show that this leads to improved distribution of the probability mass in $\tilde P$ and lower regret. 
In the space of transition functions, we will impose the constraints $\bigl|\tP_{t}(x'|x,a) - \wh{P}_{t}(x'|x,a)\bigr| \le B_{t}(x,a,x')$ for each $x'$ with $B_{t}$ defined as
\begin{equation}\label{eq:Bwidth}
 B_{t}(x,a,x') = 
 \sqrt{\frac{\wh{P}_{t}(x'|x,a)(1-\hP_{t}(x'|x,a)) \log(SAT/\delta)}{N^+_{t}(x,a)}} + \frac{???}{N^+_{t}(x,a)}. 
\end{equation}
This can be written in our framework by defining $S$ constraint aggregation functions corresponding to each state $x'$ as $w_{x'}(x) = \II{x=x'}$ for all $x$, and the corresponding confidence width $b_{x'}(x,a) = B_{t}(x,a,x')$. 
We refer to the algorithm derived from the optimistic LP with these bonuses as Bernstein OLP, or BOLP. \redd{(LOL)}
The following proposition gives the form of the exploration bonus arising from the dual optimistic LP:
\begin{proposition}\label{lem:optbern}
The exploration bonus $\CB_{h,t}$ induced by BOLP is 
\begin{align*}
\text{CB}_{h,t}(x,a) &= \min_{c(x,a) \in \bR}  \bigg \{ \sum_{y \in \cS} B_{t}(x,a,y) \bigl|\beta^*_{h+1,t}(y) - c_{h,t}(x,a)\bigr| \bigg \}.
 \end{align*}
 Furthermore, for the confidence width given in Equation~\eqref{eq:Bwidth}, the exploration bonus also satisfies
 \[
  \text{CB}_{h,t}(x,a) \le \sqrt{\frac{S\log(SAT/\delta)}{N^+_{t}(x,a)}\sum_y \hP_t(y|x,a) \Bpa{\beta_{h+1,t}^*(y) - \sum_{y'} \hP_t(y'|x,a) \beta_{h+1,t}^*(y')}^2 } + \frac{H??}{N^+_{t}(x,a)}.
 \]
\end{proposition}
\begin{proof}
For the proof of the first part, we refer to Appendix~\ref{app:}. The second half of the statement follows from setting $c_{h,t}(x,a) = \sum_{y'} \hP(y'|x,a) \beta_{h+1,t}^*(y')$, plugging in the choice of $B_{h,t}$ and using Jensen's inequality:
\begin{align*}
 &\sum_{y \in \cS} B_{t}(x,a,y) |\beta^*_{h+1,t}(y) - c_{h,t}(x,a)| 
 \\
 &\le \sum_y \sqrt{\frac{\log(SAT/\delta)}{N^+_{t}(x,a)}\hP_t(y|x,a) \Bpa{\beta_{h+1,t}^*(y) - c_{h,t}(x,a)}^2} + \frac{H??}{N^+_{h,t}(x,a)}
 \\
 &\le \sqrt{\frac{S\log(SAT/\delta)}{N^+_t(x,a)} \sum_y \hP_t(y|x,a) \Bpa{\beta_{h+1,t}^*(y) - \sum_{y'} \hP_t(y'|x,a) \beta_{h+1,t}^*(y')}^2} + \frac{H??}{N^+_{t}(x,a)}.
\end{align*}
\end{proof}
Similarly as in the previous section, we can point out a remarkable similarity between the above exploration bonus and the one used by the advanced version of UCB-VI (UCB-VI-BF, \citealp{azar2017minimax}): once again, our confidence intervals are wider by a factor of $\sqrt{S}$. Accordingly, BOLP achieves an improvement identical to what UCB-VI-BF achieves over UCB-VI-CH, in that it shaves off a factor of $\sqrt{H}$ from the regret bound of UCRL2. This is stated formally in the following proposition:
\begin{proposition}\label{prop:bolp}
The regret of BOLP satisfies
\[
\E[\Reg_T] \leq \widetilde O (S \sqrt{HAT}).
\] 
\end{proposition}
The complete proof is given in Appendix~\ref{app:}.



\subsection{Optimistic linear programming with structured constraint aggregation}
The two previous approaches using optimistic transition functions suffer from an additional $\sqrt{S}$ term in the regret compared to the lower bound. This is in contrast with the results achieved by UCB-VI \citep{azar2017minimax} and UBEV \citep{DLB17} that are both optimal in terms of their dependence on $S$. Similar results are achieved by \citet{KWY18}, \citet{ZB19} and \citet{ZJ19}. All these algorithms are either only expressed in the space of value functions, or use sophisticated confidence sets expressed in terms of some interplay between the estimated optimal value function and the transition model. We are not aware of any algorithm working purely in the space of MDPs that would successfully
\footnote{While such results are indeed claimed in the very recent work of \cite{tossou2019near}, we believe that their analysis suffers from some serious technical issues. Nevertheless, this work includes valuable ideas that have in fact inspired some of the techniques in this section.} 
remove the extra $\sqrt{S}$ factor present in the bound of UCRL2. In what follows, we describe an algorithm in our optimistic LP framework and show that it achieves a regret bound of order $H\sqrt{SAT}$.

\redd{Our approach is motivated by the observation that UCRL2 tends to select MDPs that are not statistically plausible, even though they are contained in the prescribed confidence sets. In particular, UCRL2 typically chooses a transition function $\tP_t$ such that, for a fixed $(x,a)$, $\tP_t(x'|x,a) = \tP_t(x'|x,a)$ for all but one follow-up state $x^*$, where $|\tP_t(x^*|x,a) - \hP_t(x^*|x,a)| = \varepsilon_t(x,a)$. However, Hoeffding's inequality implies that $|P(x^*|x,a) - \hP_t(x^*|x,a)| > \varepsilon_t(x,a)$ occurs with probability at most $\delta^S$, rendering the resulting transition function very unlikely to be close to $\tP_t$.}
Our approach is to construct a set of constraints that prevents the optimistic planner from putting too much probability mass on highly unlikely outcomes. For defining our constraints, we choose a fixed permutation of states all states in $\cS$ denoted as $x^{(1)},x^{(2)},\dots,x^{(S)}$ and define the subsets $\cS_i = \ev{x^{(1)},\dots,x^{(i)}}$ for all $i\in[S]$. Using the notation $P(\cS'|x,a) = \sum_{x\in\cS'} P(x'|x,a)$ for any subset $\cS'$ of $\cS$, we prescribe our confidence set in the space of transition functions as follows:
\begin{align}
 \cP_t =  \bigg\{ P\in \DeltaSSA:  \bigl|P(\cS_i|x,a) - \hP_t(\cS_i|x,a)\bigr| \leq \sqrt{ \frac{\log(2SAT/\delta)}{N^+_{t}(x,a)}} \quad \forall i \in[S] \bigg\}. \label{eqn:Pdefsubset}
 \end{align}
 It is easy to see that these constraints always assign the probability mass in a more statistically plausible way than UCRL2 does. In order to ensure that all confidence intervals hold, we take a union bound over all $S$ subsets being considered, which results in a mild blowup of order $\log S$ in the confidence widths.\footnote{The algorithm of \citet{tossou2019near} is based on a very similar idea, but they consider \emph{all subsets} of $\cS$ instead of a single sequence of nested sets. Unfortunately, using this many constraints calls for another union bound over a set of size $2^S$ which their analysis omits.}
These constraints can be expressed in our framework by using the constraint-aggregation functions $w_i(x) = \II{x\in\cS_i}$ and $b_i(x,a) = \omega_t(x,a) = \sqrt{ \log(2SAT/\delta)/N^+_{t}(x,a)}$. We refer to the algorithm resulting from solving the resulting optimistic LP as ``carefully optimistic linear programming'', or COLP. \redd{[[[sigh]]]}
Our main result regarding this algorithm is the following expression for the exploration bonus:
\begin{theorem}
 The exploration bonus $\CB_{h,t}$ induced by COLP is 
 \[
  \CB_{h,t}(x,a) = \min_{c(x,a) \in \bR}  \bigg \{\bigl|\beta^*_{h+1,t}(x^{(i^+)}) - c_{h,t}(x,a)\bigr| \bigg \} \cdot \omega_{t}(x,a),
 \]
 where $i^+\in[S]$ is an index that depends only on the function $\beta^*_{h+1,t}$.
\end{theorem}
It is easy to see that the above exploration bonus is upper-bounded by $H\omega_t(x,a)$, which precisely matches the order of the bonus used by UCB-VI-CH \citep{azar2017minimax} and UBEV \citep{DLB17}. Accordingly, we show that it achieves the following bound on the regret:
\begin{theorem}
The regret of COLP satisfies  
\[
 \Reg_T = \wt{O}(H\sqrt{SAT}).
\]
\end{theorem}
In view of the above bound, COLP can be seen to be the first optimistic RL algorithm that is defined directly in the space of MDPs and achieves the optimal dependence on the number of states $S$. Once again, its analysis is largely facilitated by the ability to separate probabilistic statements from the task of bounding the cumulative confidence widths. 

\redd{What is $i^+$ though? Can we maybe show that this algorithm will also blow its entire budget on the single largest $\beta^*_{h+1,t}$? If that's true, then the algorithm does not depend on the ordering of the states at all!!}


\section{Conclusion}

\newpage





